Characterisation of 92 Southern TESS Candidate Planet Hosts and a New Photometric [Fe/H] Relation for Cool Dwarfs

We present the results of a medium resolution optical spectroscopic survey of 92 cool ($3,000 \lesssim T_{\rm eff} \lesssim 4,500\,$K) southern TESS candidate planet hosts, and describe our spectral fitting methodology used to recover stellar parameters. We quantify model deficiencies at predicting optical fluxes, and while our technique works well for $T_{\rm eff}$, further improvements are needed for [Fe/H]. To this end, we developed an updated photometric [Fe/H] calibration for isolated main sequence stars built upon a calibration sample of 69 cool dwarfs in binary systems, precise to $\pm0.19\,$dex, from super-solar to metal poor, over $1.51 < {\rm Gaia}~(B_P-R_P) < 3.3$. Our fitted $T_{\rm eff}$ and $R_\star$ have median precisions of 0.8% and 1.7%, respectively and are consistent with our sample of standard stars. We use these to model the transit light curves and determine exoplanet radii for 100 candidate planets to 3.5% precision and see evidence that the planet-radius gap is also present for cool dwarfs. Our results are consistent with the sample of confirmed TESS planets, with this survey representing one of the largest uniform analyses of cool TESS candidate planet hosts to date.

==> tables/appendices_short.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Observations}

\begin{table}
\caption{Observing log for TESS candidate exoplanet host stars. Full table is available online as supplementary material.}
\label{tab:observing_log_tess}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Stellar Standards}\label{sec:standards}

\begin{table}
\caption{Observing log for cool dwarf standards. Full table is available online as supplementary material.}
\label{tab:observing_log_std}
\end{table}

\begin{table}
\caption{Final results for cool dwarf standards. Full table is available online as supplementary material.}
\label{tab:final_results_std}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Photometric [Fe/H] Data}

\begin{table}
\caption{Stellar pairs and primary [Fe/H] used for photometric [Fe/H] relation. Collated by \citet{mann_spectro-thermometry_2013} from \citealt{mishenina_correlation_2004}, \citealt{valenti_spectroscopic_2005}, \citealt{bean_accurate_2006}, \citet{ramirez_oxygen_2007}, \citealt{robinson_n2k_2007}, \citet{fuhrmann_nearby_2008}, \citet{casagrande_new_2011}, \citealt{da_silva_homogeneous_2011}, and \citealt{mann_spectro-thermometry_2013}. Full table is available online as supplementary material.}
\label{tab:cpm_feh}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Limb Darkening}

\begin{table}
\caption{Nonlinear limb darkening coefficients from \citet{claret_limb_2017}. Full table is available online as supplementary material.}
\label{tab:ld_coeff}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Literature Planets}

\begin{table}
\caption{Summary of literature properties for already confirmed planets. Sourced from \citet{hartman_hats-6b_2015}, \citet{esposito_gaps_2017}, \citet{bayliss_ngts-1b_2018}, \citet{gunther_super-earth_2019}, \citet{kostov_l_2019}, \citet{luque_planetary_2019}, \citet{ment_second_2019}, \citet{vanderspek_tess_2019}, \citet{winters_three_2019} \citet{dreizler_carmenes_2020}, \citet{gilbert_first_2020}, \citet{hartman_hats-47b_2020}, \citet{huang_tess_2020}, \citet{nielsen_three_2020}, \citet{waalkes_toi_2020}, and \citet{leleu_six_2021}. Full table is available online as supplementary material.}
\label{tab:planet_lit_params}
\end{table}

==> tables/table_final_results_tess_short.tex <==
\begin{table*}
\centering
\caption{Final results for TESS candidate exoplanet hosts. Full table is available online as supplementary material.}
\label{tab:final_results_tess}
\begin{tabular}{ccccccccccc}
\hline
TOI & TIC & $T_{\rm eff}$ & $\log g$ & [Fe/H] & $M$ & $R_\star$ & $m_{\rm bol}$ & $f_{\rm bol}$ & EW(H$\alpha$) & $\log R^{'}_{\rm HK}$ \\
 &  & (K) &  &  & ($M_\odot$) & ($R_\odot$) &  & {{\footnotesize(10$^{-12}\,$ergs s$^{-1}$ cm $^{-2}$)}} & \SI{}{\angstrom} &  \\
\hline
136 & 410153553 & 2988 $\pm$ 30 & 5.06 $\pm$ 0.02 &- &0.155 $\pm$ 0.004 &0.192 $\pm$ 0.004 &12.05 $\pm$ 0.01 &384.4 $\pm$ 3.9 &-0.05 & -5.37 \\
540 & 200322593 & 3104 $\pm$ 30 & 5.07 $\pm$ 0.02 &-0.10 &0.164 $\pm$ 0.004 &0.197 $\pm$ 0.004 &11.71 $\pm$ 0.01 &528.3 $\pm$ 5.3 &2.49 & - \\
256 & 92226327 & 3150 $\pm$ 30 & 5.01 $\pm$ 0.02 &-0.13 &0.182 $\pm$ 0.005 &0.220 $\pm$ 0.004 &11.55 $\pm$ 0.01 &611.8 $\pm$ 6.1 &-0.22 & -5.53 \\
203 & 259962054 & 3169 $\pm$ 30 & 5.01 $\pm$ 0.02 &-0.07 &0.200 $\pm$ 0.005 &0.232 $\pm$ 0.004 &12.49 $\pm$ 0.01 &255.4 $\pm$ 2.6 &0.56 & -4.98 \\
507 & 348538431 & 3279 $\pm$ 30 & 4.76 $\pm$ 0.02 &- &0.383 $\pm$ 0.010 &0.424 $\pm$ 0.008 &14.28 $\pm$ 0.01 & 49.2 $\pm$ 0.5 &2.24 & -4.49 \\
910 & 369327947 & 3282 $\pm$ 30 & 4.97 $\pm$ 0.02 &-0.04 &0.262 $\pm$ 0.008 &0.278 $\pm$ 0.005 &10.46 $\pm$ 0.01 &1656.2 $\pm$ 16.6 &-0.27 & -5.47 \\
210 & 141608198 & 3284 $\pm$ 30 & 4.90 $\pm$ 0.02 &0.21 &0.312 $\pm$ 0.008 &0.326 $\pm$ 0.006 &12.78 $\pm$ 0.01 &195.8 $\pm$ 2.0 &-0.23 & -5.84 \\
122 & 231702397 & 3326 $\pm$ 30 & 4.86 $\pm$ 0.02 &-0.07 &0.316 $\pm$ 0.008 &0.345 $\pm$ 0.006 &13.42 $\pm$ 0.01 &109.3 $\pm$ 1.1 &-0.21 & - \\
455 & 98796344 & 3330 $\pm$ 30 & 4.97 $\pm$ 0.02 &-0.27 &0.248 $\pm$ 0.006 &0.271 $\pm$ 0.005 &9.16 $\pm$ 0.01 &5507.5 $\pm$ 54.8 &-0.29 & -5.39 \\
732 & 36724087 & 3354 $\pm$ 30 & 4.83 $\pm$ 0.02 &0.13 &0.364 $\pm$ 0.009 &0.382 $\pm$ 0.007 &10.91 $\pm$ 0.01 &1103.5 $\pm$ 11.0 &-0.23 & -5.55 \\
\hline
\end{tabular}
\end{table*}


==> tables/table_planet_params_short.tex <==
\begin{table*}
\centering
\caption{Final results for TESS candidate exoplanets. Full table is available online as supplementary material.}
\label{tab:planet_params}
\begin{tabular}{ccccccccc}
\hline
TOI & TIC & Sector/s & Period & $R_p/R_{\star}$ & $a/R_{\star}$ & $e$ flag & $i$ & $R_p$ \\
 &  &  & (days) &  &  &  & ($^{\circ}$) & ($R_{\oplus}$) \\
\hline
122.01 & 231702397 & 1,27-28 & 5.07803 $\dagger$ &0.0797 $\pm$ 0.0022 &24.63 $\pm$ 0.49 &0 & 88.337 $\pm$ 0.001 &3.00 $\pm$ 0.10\\
129.01 & 201248411 & 1-2,28-29 & 0.98097 $\dagger$ &0.3223 $\pm$ 0.0884 &5.15 $\pm$ 0.04 &0 & 76.381 $\pm$ 0.018 &25.35 $\pm$ 6.96\\
133.01 & 219338557 & 1,28 & 8.19918 $\dagger$ &0.0269 $\pm$ 0.0010 &23.15 $\pm$ 0.41 &0 & 88.470 $\pm$ 0.002 &1.88 $\pm$ 0.07\\
134.01 & 234994474 & 1,28 & 1.40153 $\dagger$ &0.0223 $\pm$ 0.0006 &6.98 $\pm$ 0.16 &0 & 84.566 $\pm$ 0.005 &1.54 $\pm$ 0.05\\
136.01 & 410153553 & 1,27-28 & 0.46293 $\dagger$ &0.0587 $\pm$ 0.0006 &6.80 $\pm$ 0.17 &1 & 90.000 $\pm$ 5.000 &1.23 $\pm$ 0.03\\
139.01 & 62483237 & 1,28 & 11.07083 $\dagger$ &0.0346 $\pm$ 0.0008 &27.20 $\pm$ 0.56 &0 & 88.549 $\pm$ 0.001 &2.54 $\pm$ 0.07\\
142.01 & 425934411 & 1-2,28-29 & 0.85335 $\dagger$ &0.1809 $\pm$ 0.0184 &4.74 $\pm$ 0.11 &0 & 79.385 $\pm$ 0.012 &13.31 $\pm$ 1.39\\
175.01 & 307210830 & 2,5,8-12,28-29,32 & 3.69066 $\dagger$ &0.0397 $\pm$ 0.0003 &21.32 $\pm$ 0.47 &0 & 88.809 $\pm$ 0.002 &1.32 $\pm$ 0.03\\
175.02 & 307210830 & 2,5,8-12,28-29,32 & 7.45075 $\dagger$ &0.0446 $\pm$ 0.0006 &34.59 $\pm$ 0.75 &0 & 88.483 $\pm$ 0.001 &1.48 $\pm$ 0.03\\
175.03 & 307210830 & 2,5,8-12,28-29,32 & 2.25310 $\dagger$ &0.0238 $\pm$ 0.0003 &15.76 $\pm$ 0.34 &0 & 88.133 $\pm$ 0.003 &0.79 $\pm$ 0.02\\
\hline
\end{tabular}
\begin{minipage}{\linewidth}
\vspace{0.1cm}
\textbf{Notes:} Periods denoted by $\dagger$ are not as reported by ExoFOP, and have been refitted here. These are overwhelmingly systems with TESS extended mission data, thus having longer time baselines with which to constrain orbital periods. Our fitted periods however are generally consistent within uncertainties of their ExoFOP values, and as such we do not report new uncertainties here. Additionally, our least squares fits to 7 of our light curves proved insenstive to non-edge-on inclinations. As such, we report conservative uncertanties of $\pm5$\degree~ for these planets.\\
\end{minipage}
\end{table*}

